Do I Belong? Modeling Sense of Virtual Community Among Linux Kernel Contributors

The sense of belonging to a community is a basic human need that impacts an individuals behavior, long-term engagement, and job satisfaction, as revealed by research in disciplines such as psychology, healthcare, and education. Despite much research on how to retain developers in Open Source Software projects and other virtual, peer-production communities, there is a paucity of research investigating what might contribute to a sense of belonging in these communities. To that end, we develop a theoretical model that seeks to understand the link between OSS developer motives and a Sense of Virtual Community. We test the model with a dataset collected in the Linux Kernel developer community, using structural equation modeling techniques. Our results for this case study show that intrinsic motivations - social or hedonic motives - are positively associated with a sense of virtual community, but living in an authoritative country and being paid to contribute can reduce the sense of virtual community. Based on these results, we offer suggestions for open source projects to foster a sense of virtual community, with a view to retaining contributors and improving projects sustainability.

==> Tables/cluster.tex <==
\begin{table}[!b]
\centering
\caption{Group Paths Coefficients (bold are significant p values)}
\label{tab:cluster}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{P{2.8cm}
                S[table-format=0.2]
                S[table-format=0.2]
                S[table-format=0.2]
                S[table-format=0.2]}

\toprule


& {\makecell{Social\\motives}} & {\makecell{All\\motives}} & {\makecell{Non\\Hedonists}} & {Hedonists} \\ \midrule
\hangindent1em (H1) Social motives $\rightarrow$ SVC & \bfseries .18 & \bfseries .30 & \bfseries .31 & .04 \\ 
%\hline
\addlinespace 
\hangindent1em (H2) Hedonic motives$\rightarrow$SVC & .07 & \bfseries .45 & -.08 & \bfseries .51 \\ 
%\hline
\addlinespace 
\hangindent1em (H3) Moral motives$\rightarrow$SVC & -.02 & \bfseries -.18 & -.23 & -.08 \\ 
%\hline
\addlinespace 


\hangindent1em (H4a) Power distance \texttimes{} Social motives $\rightarrow$ SVC & \bfseries -.23 & \bfseries .15 & \bfseries -.46 & \bfseries -.25 \\ 
%\hline
\addlinespace 
\hangindent1em (H4b) Power distance \texttimes{} Hedonic motives $\rightarrow$SVC & {-.03} & .07 & {.00} & .05 \\ 
%\hline
\addlinespace 
\hangindent1em (H4c) Power Distance \texttimes{} Moral motives$\rightarrow$SVC & -.07 & -.06 & .08 & \bfseries .29 \\ 
%\hline
\addlinespace 
\hangindent1em (H5a) Is paid \texttimes{} Social motives$\rightarrow$SVC & {{.72}} & {-.04} & {{-.50}} & \bfseries -.24  \\ 
%\hline
\addlinespace 
\hangindent1em (H5b) Is paid \texttimes{} Hedonic motives$\rightarrow$SVC & \bfseries -.20 & \bfseries .19  & \bfseries -.26 & \bfseries .17 \\ 
%\hline
\addlinespace 
\hangindent1em (H5c) Is paid \texttimes{} Moral motives$\rightarrow$SVC & {.02} & .06 &\bfseries .17 & \bfseries .28 \\ 
%\hline
%\addlinespace 
\midrule
Control variables\\
\midrule
Tenure$\rightarrow$SVC & \bfseries .27 & \bfseries .11 & \bfseries .45 & .04 \\ 
%\hline
\addlinespace 
\hangindent1em Gender minorities$\rightarrow$SVC & \bfseries -.22 & \bfseries -.19 & \bfseries -.30 & \bfseries -.27 \\ 
%\hline
\addlinespace 
\hangindent1em English confidence$\rightarrow$SVC & .00 & \bfseries .59 & -.03 & \bfseries .70 \\ 




\bottomrule


\end{tabular}
\end{table}

==> Tables/cluster_new_2_segments.tex <==
\begin{table}[!b]
\centering
\caption{Group Paths Coefficients (bold are significant p values)}
\label{tab:cluster_new}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{P{5.4cm}
                S[table-format=0.2]
                S[table-format=0.2]}

\toprule


%& {\makecell{Power\\ Distance \\ (n=182) \\ \textit{R}\textsuperscript{2} 0.519}} & {\makecell{No Power\\ Distance \\ (n=225) \\  \textit{R}\textsuperscript{2} 0.396} } \\ 
& {\makecell{Power \\Distance}} & {\makecell{No Power \\Distance}}\\
\midrule
Sample size (N) & {182} & {225}\\
\addlinespace
Coefficient of determination (\textit{R}\textsuperscript{2}) & .519 & .396\\
%\addlinespace
\midrule 
\hangindent1em (H1) Social motives $\rightarrow$ SVC & \bfseries .37 & \bfseries .25 \\ 
%\hline
\addlinespace 
\hangindent1em (H2) Hedonic motives$\rightarrow$SVC & \bfseries.48 & \bfseries .42 \\ 
%\hline
\addlinespace 
\hangindent1em (H3) Moral motives$\rightarrow$SVC & -.16 &  -.14 \\ 
%\hline
\addlinespace 


\hangindent1em (H4a) Power distance \texttimes{} Social motives $\rightarrow$ SVC & -.13 & \bfseries-.15 \\ 
%\hline
\addlinespace 
\hangindent1em (H4b) Power distance \texttimes{} Hedonic motives $\rightarrow$SVC & -.10 & -.05 \\ 
%\hline
\addlinespace 
\hangindent1em (H4c) Power Distance \texttimes{} Moral motives$\rightarrow$SVC & -.07 & .04 \\ 
%\hline
\addlinespace 
\hangindent1em (H5a) Is paid \texttimes{} Social motives$\rightarrow$SVC & -.10 & -.05  \\ 
%\hline
\addlinespace 
\hangindent1em (H5b) Is paid \texttimes{} Hedonic motives$\rightarrow$SVC & \bfseries -.42 & \bfseries -.33 \\ 
%\hline
\addlinespace 
\hangindent1em (H5c) Is paid \texttimes{} Moral motives$\rightarrow$SVC & .17 & .12 \\ 
%\hline
%\addlinespace 
\midrule 
Tenure$\rightarrow$SVC & \bfseries .38 & \bfseries .28 \\ 
%\hline
\addlinespace 
\hangindent1em Gender minorities$\rightarrow$SVC & \bfseries -.55 & \bfseries -.50 \\ 
%\hline
\addlinespace 
\hangindent1em English confidence$\rightarrow$SVC &  \bfseries .16 & \bfseries .13 \\ 

\hline
\addlinespace 
\hangindent1em is Paid$\rightarrow$SVC &  \bfseries .24 & \bfseries .42 \\ 

%\hline
\addlinespace 
\hangindent1em Power distance$\rightarrow$SVC  & \bfseries -.17 & .07 \\ 

\bottomrule


\end{tabular}
\end{table}

==> Tables/cronbach_cr.tex <==
\begin{table}[!b]
\centering
\caption{Internal Consistency Reliability}
\label{tab:internal_consistency_reliability}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=3, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{p{3.2cm}
                S
                S
                S}
\toprule
& {\makecell{Cronbach's \textalpha}} & {\makecell{CR}} & {AVE}\\
\midrule
English Confidence & .932 & .951 & .830\\
%\midrule
%\addlinespace
Sense of Virtual Community & .767 & .839 & .511\\
\bottomrule


\end{tabular}
\end{table}

==> Tables/discussion.tex <==
\begingroup
%% I removed the hyp numbers because the encoding of those characters must have been messed up as I spent a good while fixing errors. Perhaps have to retype them.

\footnotesize
\begin{longtable}[h]{p{2.5cm}p{4.5cm}p{4cm}}
\caption{Summary of results and implications}\label{tab:discussion}\\
\toprule
Hypotheses&Findings&Implications\\
\midrule
\endfirsthead
\multicolumn{3}{l}{{Table~\thetable{} continued}}\\
\toprule
Hypotheses&Findings&Implications\\
\midrule
\endhead
\bottomrule
\multicolumn{3}{c}{continued on next page}\\
\endfoot
\endlastfoot

%%%Social aspects (e.g., altruism, kinship, and reputation) have gone up in the ranking [ICSE MOTIVATION]
%%%The  frequency  of  mentions  to Altruism also  increased,  from  18.0%  to  26.7%. Reputation,Kinship, and Reciprocity also had noticeable increases. [ICSE MOTIVATION]
%%% Social and philosophical  factors  (such  as Ideology and Altruism)  as well as Pay are reported more often by experienced developers
%%Whereas ideology, own-use or education-related programs can be an impetus to  join  OSS,  individuals  con-tinue  for  intrinsic  reasons  (fun,  altruism,  reputation,  andkinship)
H1. Kinship, Altruism $\rightarrow$ SVC & Supported. While the standardized path coefficient was moderate (0.2), contributors from our sample who are motivated by Kinship or Altruism have a positive association with the sense of virtual community.
%though the effect size is low (.042) 
& The intrinsic-social motivations of kinship and altruism are associated with the sense of virtual community. Besides online interest groups for members, chat rooms, instant messaging, and discussion forums to encourage community involvement \citep{xu2015empirical}, OSS communities can provide online tools with shared spaces for contributors to work ``together" on issues, discuss and collaborate on similar interests. Better interactions can strengthen contributors’ Sense of Virtual Community, especially for those who seek social relationships. 
\\
%\midrule
\addlinespace
%%%The  odds  of Fun motivating  coders  were  4x  higher  than non-coders
%%% Most of the OSS contributors who participated on Gerosa et al (2021)’s study (91%)
%%% Researchers: ir além de aspectos técnicos e entender mais a fundo o quão entertaining os projetos são, etc...
%multidimension of flourishing
%%https://papers.ssrn.com/sol3/papers.cfm?abstract_id=957174 (happiness / volunteering)
%%%Happiness --> Graziotin
%agreed (or strongly agreed) that they contribute to OSS due to entertainment (fun)
H2. Fun $\rightarrow$ SVC & Supported. Although the standardized path coefficient was moderate (0.2), contributors motivated by Enjoyment, Hobby, or Fun have a positive association with the Sense of Virtual Community.
%though the effect size is small (0.059).
& OSS communities should create an enjoyable environment and take actions to mitigate the toxicity that repeals contributors motivated by the excitement of making contributions \citep{raman2020stress,cohen2021contextualizing,miller2022did}.

\\
%\midrule
\addlinespace

H3. Ideology, Reciprocity $\rightarrow$ SVC & Not supported. Being motivated by Ideology or Reciprocity does not associate with a higher Sense of Virtual Community (standardized path coefficient 0.06, p 0.372). &
%Considering that contributors who join by Ideology often shift to other motivations \cite{gerosa2021shifting}, communities should offer opportunities for them to develop other motivations that can help foster a Sense of Virtual Community.
\\ 
%\midrule
\addlinespace

%%% 
H4a. Power Distance X Kinship, Altruism $\rightarrow$ SVC & Weak Support. 
Being surrounded by a country culture with high levels of power distance has a low standardized path coefficient (-0.160) with a marginally significant p-value of 0.053 (following the standard alpha level of 0.05).
%with a small effect size (.023)
& 
Being marginally significant, the results align with Cognitive Theory \citep{deci1985cognitive} on the fact that contributors motivated by Kinship or Altruism need more autonomy (through less hierarchy) to develop a Sense of Virtual Community.\\
%The finding is aligned with the biosocial needs which poses that a close emotional bond (belonginess and attachment) comes together with the act of shifting the power to the learner (autonomy), and acts of altruism.
%\midrule
\addlinespace

H4b. Power Distance X Fun $\rightarrow$ SVC  & Not supported. Being surrounded by a country culture with high levels of Power Distance does not impact the association that contributors motivated by Enjoyment, Hobby, or Fun have to experience a Sense of Virtual Community (standardized path coefficient -0.047, p 0.548). & 
%Levels of autonomy did not cause any effect on the positive association of contributors motivated by Enjoyment, Hobby, or Fun and the Sense of Virtual Community. 
\\
%Future research is needed to evaluate in which details the autonomy is relevant for those contributors.
 %\midrule
 \addlinespace
H4c. Power Distance X Ideology, Reciprocity $\rightarrow$ SVC & Not supported. Being surrounded by a country culture with high levels of Power Distance does not impact the association that contributors motivated by Ideology or Reciprocity have to experience a Sense of Virtual Community (standardized path coefficient 0.035, p = 0.647). & %Levels of autonomy did not made any difference to contributors motivated by Ideology or Reciprocity and their Sense of Virtual Community.
\\
 %\midrule
 \addlinespace
 
H5a. Is Paid X Kinship, Altruism $\rightarrow$ SVC & Not supported. Being paid or a volunteer does not impact the association that contributors motivated by Kinship or Altruism have to experience a Sense of Virtual Community (standardized path coefficient 0.029, p 0.679). & 
%Being paid to contribute does not cause any effect on the positive association of contributors motivated by the social-intrinsic motivations of Kinship or Altruism and the Sense of Virtual Community. Future research can evaluate if the social bond that contributors driven by Kinship or Altruism make with the community is stronger than compensation to influence their decision to stay in the project even not being paid or receiving a job offer to move to another project.
\\
% \midrule
H5b. Is Paid X Fun $\rightarrow$ SVC & Supported. When being paid, contributors motivated by Enjoyment, Hobby, or Fun have a reverse association with the Sense of Virtual Community (standardized path coefficient -0.15, p 0.048). Hence, those contributors are less likely to experience a sense of virtual community.
%though the effect size is low (0.025). 
&  Even enjoying contributing to the Linux Kernel, paid contributors showed a lower Sense of Virtual Community to the Linux Kernel. This result is aligned with the Cognitive Theory \citep{deci1985cognitive} and can be explained by the conflicting identities and hybrid belonging paid contributors have to both their sponsoring firms and the Linux Kernel community. \\
%OSS community should focus strategies to foster a sense of virtual community in order to retain people who are paid to do their work but also feel the excitement and the joy of contributing
 %\midrule
 \addlinespace
H5c. Is Paid X Ideology, Reciprocity $\rightarrow$ SVC  & Not supported. Being paid or a volunteer does not impact the association that contributors motivated by ideology or reciprocity have to experience a sense of virtual community (standardized path coefficient .035, p .647). & 
%Being intrinsically motivated by Ideology or Reciprocity, independently of the contributor's compensation, have no association with a Sense of Virtual Community. More research is necessary to find ways to entice contributors who are driven by those motivations to develop a sense of virtual community.
\\ 
% \midrule
% \multicolumn{3}{l}{Control Variables}\\
% \midrule
%Gender Minorities$\rightarrow$SVC & Contributors in gender minorities tend to experience lower levels of sense of virtual community (standardized path coefficient -.137, p .027), though the effect size is low (.028) & xxx\\ 
 %\midrule
% \addlinespace
%English Confidence$\rightarrow$SVC & Contributors with higher levels of English confidence tend to experience higher levels of sense of virtual community (standardized path coefficient 0.144, p 0.019), though the effect size is low (.026). & xxx\\ 
 %\midrule
% \addlinespace
%Tenure$\rightarrow$SVC & Over the time, contributors tend to experience higher levels of sense of virtual community (standardized path coefficient .252, p .000), though the effect size is low (.081). & xxx\\

\bottomrule
\end{longtable}
\endgroup

==> Tables/effect_size.tex <==
\begin{table}[htb]
\centering
\caption{Effect sizes for all constructs (with specified endogenous variable to which the effect size applies)}
\label{tab:effect_size}

\sisetup{
    table-format=1.3,
    mode=text,
    detect-weight=true, 
    detect-family=true,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=3 %% change this for precision.
}
\begin{tabular}{p{7cm}S}
\toprule
{Hypotheses} & {\textit{f}\textsuperscript{2}}\\
\midrule

(H1) Kinship, Altruism $\rightarrow$ SVC & .042\\
\addlinespace
(H2) Fun $\rightarrow$ SVC & .059\\
\addlinespace
(H3) Ideology, Reciprocity $\rightarrow$ SVC & .004\\
\addlinespace
(H4a) Power Distance X Kinship,Altruism $\rightarrow$ SVC & 0.023\\
\addlinespace
(H4b) Power Distance X Fun $\rightarrow$ SVC  & .003 \\
\addlinespace
(H4c) Power Distance X Ideology, Reciprocity $\rightarrow$ SVC & .002\\
\addlinespace
(H5a) Is paid X Kinship $\rightarrow$ SVC & .001  \\ 
\addlinespace
(H5b) Is paid X Fun $\rightarrow$ SVC & .025  \\ 
\addlinespace
(H5c) Is paid X Ideology $\rightarrow$ SVC & .001 \\ 
\midrule
\textsc{Control Variables}&\\
\midrule 
Gender Minorities $\rightarrow$ SVC    & .028 \\ 
\addlinespace
English Confidence $\rightarrow$ SVC & .026 \\ 
\addlinespace
Tenure $\rightarrow$ SVC & .081\\
\bottomrule
\end{tabular}

%\resizebox{0.7\textwidth}{!}{%
%\begin{tabular}{|ll|}
%\hline
%\multicolumn{1}{|l|}{}                                                              & {\cellcolor[HTML]{C0C0C0}\textbf{Effect Sizes}} \\ \hline
%\multicolumn{2}{|l|}{\textbf{Hypotheses}}                                                                   \\ \hline
%\multicolumn{1}{|l|}{(H1) Kinship/Altruism \rightarrow SVC} & 0.042 \\ \hline
%\multicolumn{1}{|l|}{(H2) Fun \rightarrow SVC} & 0.059 \\ \hline
%\multicolumn{1}{|l|}{(H3) Ideology/Reciprocity \rightarrow SVC} & 0.004 \\ \hline
%\multicolumn{1}{|l|}{(H4a) Power Distance X Kinship/Altruism \rightarrow SVC} & 0.023  \\ \hline
%\multicolumn{1}{|l|}{(H4b) Power Distance X Fun \rightarrow SVC} & 0.003 \\ \hline
%\multicolumn{1}{|l|}{(H4c) Power Distance X Ideology/Reciprocity \rightarrow SVC}  & 0.002 \\ \hline
%\multicolumn{1}{|l|}{(H5a) Is paid X Kinship/Altruism \rightarrow SVC} & 0.001 \\ \hline
%\multicolumn{1}{|l|}{(H5b) Is paid X Fun \rightarrow SVC}                         & 0.025 \\ \hline
%\multicolumn{1}{|l|}{(H5c) Is paid X Ideology/Reciprocity \rightarrow SVC}                    & 0.001                 \\ \hline
%\multicolumn{2}{|l|}{\textbf{Control Variables}}                                                            \\ \hline
%\multicolumn{1}{|l|}{Gender Minorities \rightarrow SVC}                           & 0.028 \\ \hline
%\multicolumn{1}{|l|}{English confidence \rightarrow SVC}                         & 0.026 \\ \hline
%\multicolumn{1}{|l|}{Tenure \rightarrow SVC}                                    & 0.081 \\ \hline
%\end{tabular}}

\end{table}

==> Tables/fornell-larcker.tex <==
\begin{table}[htb]
\centering
\caption{Fornell-Larcker criterion: correlations among the constructs and square roots of the AVE values (on diagonal) [see source comment]}
\label{tab:fornell-larcker}

\begin{tabular}{p{5cm}p{1.3cm}p{1.3cm}}
\toprule
&English Confidence & SVC\\
\midrule
English Confidence & \textbf{0.909} & \\
\addlinespace
Sense of Virtual Community & 0.253 & \textbf{0.710}\\
\bottomrule

%\begin{tabular}{ll|l|l|}
%&{\cellcolor[HTML]{C0C0C0}English confidence} & {\cellcolor[HTML]{C0C0C0}SVC} \\ \hline
%{\cellcolor[HTML]{C0C0C0}English confidence} & \textbf{0.909}      &                \\ \hline
%{\cellcolor[HTML]{C0C0C0}SVC}                 & 0.253               & \textbf{0.710} \\ \hline


\end{tabular}
\end{table}

==> Tables/new_fornell_larcker.tex <==
\begin{table}[htb]
\centering
\caption{Fornell-Larcker criterion: correlations among the constructs and square roots of the AVE values (on diagonal)}
\label{tab:new_fornell_larcker}
\robustify{\bfseries}
\footnotesize

\begin{tabular}{P{1.37cm}p{0.46cm}p{0.46cm}p{0.46cm}p{0.2cm}p{0.46cm}p{0.2cm}p{0.46cm}p{0.2cm}p{0.2cm}}
\toprule
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
 \midrule
(1) English Confidence & \textbf{.91} &  &  &  &  &  &  &  &  \\ \addlinespace
(2) Fun & -.13 & \textbf{1.00} &  &  &  &  &  &  &  \\ \addlinespace
(3) Gender Minorities & .03 & -.05 & \textbf{1.00} &  &  &  &  &  &  \\ \addlinespace
(4) Ideology Reciprocity & .02 & .27 & -.08 & \textbf{1.00} &  &  &  &  &  \\ \addlinespace
(5) Is Paid & .35 & -.10 & .01 & .07 & \textbf{1.00} &  &  &  &  \\ \addlinespace
(6) Kinship Altruism & .06 & .39 & -.05 & .43 & .09 & \textbf{1.00} &  &  &  \\ \addlinespace
(7) Power Distance & -.26 & .19 & .09 & .05 & -.15 & .14 & \textbf{1.00} &  &  \\ \addlinespace
(8) SVC & .25 & .27 & -.19 & .18 & .32 & .35 & -.04 & \textbf{.71} &  \\ \addlinespace
(9) Tenure & .33 & .01 & -.17 & .08 & .25 & .12 & -.29 & .38 & \textbf{1.00}
\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/path_analysis.tex <==
\begin{table*}[!tb]
\centering
\caption{Standarized path coefficients, bootstrap estimates, standard deviations, confidence intervals, and p values}
\label{tab:path_analysis}
\robustify{\bfseries}
\sisetup{
    table-format=-1.3,
    mode=text,
    group-digits = false ,
    input-signs =- ,
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{p{6cm}SSSp{2cm}S}
\toprule
& {\textit{B}} & {Bootstrap Mean} & {SD} & {95\% CI} & {\textit{p}}\\
\midrule
\textsc{Hypotheses}&&&&&\\
\midrule
(H1) Kinship, Altruism$\rightarrow$SVC & 0.198 & 0.196 & 0.067 & (0.062,0.329) & \bfseries 0.003\\
\addlinespace
(H2) Fun$\rightarrow$SVC & 0.223 & 0.227 & 0.074 & (0.077,0.369) & \bfseries 0.003\\
\addlinespace
(H3) Ideology, Reciprocity$\rightarrow$SVC & -.060 & -0.062 & 0.067 & (-0.191,0.071) & 0.372\\
\midrule
Moderators \\
\midrule
(H4a) Power Distance \texttimes{} Kinship,Altruism $\rightarrow$ SVC\\ & -0.160 & -0.161 & 0.081 & (-0.332,-0.012) & \bfseries 0.053\\
\addlinespace
(H4b) Power Distance \texttimes{} Fun $\rightarrow$SVC  & -0.047 & -0.037 & 0.078  & (-0.188,0.115)  & 0.548 \\
\addlinespace
(H4c) Power Distance \texttimes{} Ideology, Reciprocity$\rightarrow$SVC & 0.035 & 0.031 & 0.076  & (-0.127,0.169)  & 0.647\\
\addlinespace
(H5a) Is paid \texttimes{} Kinship$\rightarrow$SVC & -0.028 & -0.026  & 0.067  & (-0.156,0.103) & 0.672  \\ 
\addlinespace
(H5b) Is paid \texttimes{} Fun$\rightarrow$SVC & -0.145 & -0.142 & 0.073 & (-0.287,0.001)  & \bfseries 0.045  \\ 
\addlinespace
(H5c) Is paid \texttimes{} Ideology$\rightarrow$SVC & 0.029 & 0.029  & 0.071  & (-0.111, 0.168) & 0.679 \\ 
\midrule
\textsc{Control Variables}&&&&&\\
\midrule
Gender Minorities$\rightarrow$SVC    & -0.137  & -0.135 & 0.062  & (-0.260,-0.015) & \bfseries 0.027 \\ 
\addlinespace
English Confidence$\rightarrow$SVC & 0.144  & 0.146   & 0.061 & (0.026,0.265) & \bfseries 0.019 \\ 
\addlinespace
Tenure$\rightarrow$SVC & 0.252  & 0.252 & 0.064 & (0.126,0.376)  & \bfseries 0.000\\

\bottomrule


%\resizebox{1\textwidth}{!}{%
%\begin{tabular}{|lccccc|}
%\hline
%\rowcolor[HTML]{C0C0C0} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}}                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Coefficient}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Bootstrap Mean}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Std.dev.}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{95\% CI}}  & \textbf{P Values} \\ \hline
%\rowcolor[HTML]{EFEFEF} 
%\multicolumn{6}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Hypotheses}}} \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H1. Kinship/Altruism $\rightarrow$ SVC}      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.198}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.196}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.067}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(0.062, 0.329)}    & 0.003             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H2. Fun $\rightarrow$ SVC}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.223}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.227}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.074}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(0.077, 0.369)}    & 0.003             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H3. Ideology/Reciprocity $\rightarrow$ SVC}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.06}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.062}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.067}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.191, 0.071)}   & 0.372             \\ \hline
          
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H4a. Power Distance X Kinship/Altruism $\rightarrow$ SVC}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.16}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.161}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.081}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.332,  -0.012)} & 0.05              \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H4b. Power Distance X Fun $\rightarrow$ SVC}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.047}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.037}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.078}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.188,  0.115)}  & 0.548             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H4c. Power Distance X Ideology/Reciprocity $\rightarrow$ SVC} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.035}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.031}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.076}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.127, 0.169)}   & 0.647             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H5a. Is paid X Kinship $\rightarrow$ SVC}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.028}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.026}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.067}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.156, 0.103)}   & 0.672             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H5b. Is paid X Fun $\rightarrow$ SVC}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.145}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.142}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.073}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.287,  0.001)}  & 0.048             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}H5c. Is paid X Ideology $\rightarrow$ SVC}                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.029}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.029}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.071}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.111,  0.168)}  & 0.679             \\ \hline
%\multicolumn{6}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{Control Variables}}}                                                                                                                              \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}Gender Minorities $\rightarrow$ SVC}                           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.137}               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}-0.135}                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.062}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(-0.260, -0.015)}  & 0.027             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}English confidence $\rightarrow$ SVC}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.144}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.146}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.061}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(0.026, 0.265)}    & 0.019             \\ \hline
%\rowcolor[HTML]{FFFFFF} 
%\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}Tenure $\rightarrow$   SVC}                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.252}                & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.252}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.064}             & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}(0.126, 0.376)}    & 0.000                 \\ \hline
%\end{tabular}}

\end{tabular}
\end{table*}

==> unused_text.tex <==
%Two respondents mentioned the sense of belonging on their motivations to be a Linux Kernel contributors, as \textit{``being part of a fantastic community"} (S178) and \textit{``makes me feel that I am a part of something big."} (S27). While that, another respondent mentioned to face challenges about \textit{``lack of sense of belonging, cultural gaps due to not being part of the in-group, not being able to relate to colleagues, sense of otherness that never goes away"} (S80). The lack of fit as opposed to the intrinsic motivations was also mentioned by another respondent: \textit{``I did not fit in, in a big way. I was never able to create enough social capital to make networking effective, no matter who I tried to connect with."} (S37) This shows the sense of virtual community in the Linux Kernel is not being achieved for people who are intrinsically motivated and want to have social capital and be part of the group. One respondent mentioned that a reason to leave could be ``the person not being a good fit for the kernel" (S138).

%Researchers have also shown that developers' turnover impacts software quality \cite{mockus2010,mockus2009, foucault2015}. To better understand how to retain contributors, \citet{lin2017developer} investigated which development activities influence continued OSS contributions and \citet{lee2002social} showed that job satisfaction strongly influences turnover intentions.
%Experienced developers are important for software projects to succeed. Projects that can retain developers for longer periods increase the knowledge base and expertise: as the productivity of newcomers increases, they acquire more experience to conduct critical tasks in the project \cite{shah2006motivation,zhou2010developer}. Once newcomers join, the project should try to keep them for extended periods of time. Projects may need six or even more newcomers to replace the productivity of a single experienced developer \cite{mockus2009succession}. The challenges people face while contributing can turn into motivations to leave and impact retention.

%A majority of newcomers (as high as 80\% in some projects) do not become long-term contributors \cite{steinmacher2013newcomers}. \citet{pinto2016more} found that almost half of the contributors of a project submit a single contribution and do not go back  \cite{pinto2016more}, and many participants never have a pull request accepted \cite{steinmacher2018almost}.} 

%High turnover has a negative impact on team cognition and performance \cite{levine2004,levine2005}, and its costs on the project and society \cite{graef2000, garman2005}. Developers' turnover harms software development projects \cite{bass2018employee, nakatsu2009comparative, hall2008}. Projects with high turnover are less successful \cite{hall2008} and projects that retain developers for longer periods increase the knowledge base and expertise \cite{shah2006motivation,zhou2010developer}. 

%Open Source Software (OSS) has become part of today's critical IT infrastructure \cite{Steinmacher.Teenager:2017}. 

%Traditionally, OSS communities consisted primarily of volunteers, but today many large projects are sponsored or maintained by companies. While corporate engagement can be a positive influence on open source projects, it can also lead to corporate dominance, which in turn may negatively affect the sustainability of an open source project \cite{zhang2022esecfse}.

%However, a majority of newcomers (as high as 80\% in some projects) do not become long-term contributors \cite{steinmacher2013newcomers}. Almost half of the contributors of a project submit a single contribution and do not go back \cite{pinto2016more}. 

%intrinsic motivation refers to undertaking action because it is inherently interesting or enjoyable while extrinsic motivation refers to activity undertaken because it leads to a separable outcome. Whereas intrinsic motivation moves one to act for satisfaction, enjoyment, or personal challenge, extrinsic motivation propels action because it is externally rewarded and valued by others to whom one is connected \cite{ryan2000self}.

%Many contributors can never have a pull request accepted \cite{steinmacher2018almost}.

%Developers' turnover impacts software quality \cite{mockus2010,mockus2009,foucault2015} and the project success \cite{hall2008}.
%Each time a newcomer joins an Open Source Software project, this person is be introduced to the community, its processes, and its culture. Typically this is done through an onboarding process.
%Moreover, onboarding programs can be insufficient if those who join do not feel that they belong to the community and ultimately abandon the project---a frequent occurrence in OSS \cite{steinmacher2013newcomers}.

%The concept of sense of belonging is related to other concepts loneliness, alienation, and social support \cite{allen2020beginnings}.  %People who lack such a sense of belonging may leave an organization \cite{davila2012organizational}. 

%Fun and ideology were the top reported motivations reported by \cite{difranzo2011farm}'s study on Windowsfarm virtual communities, who suggested more research on how to support those motivations to foster participation of virtual communities.

%We do not suggest that the concepts we use cannot also be applied to contributors driven by extrinsic motivations, and indeed it is possible that the model might prove more broadly applicable. However, we have chosen to focus on intrinsic motivations in order to produce less ambiguous results. In this paper, we contribute to the scientific body of knowledge by providing a theoretical model of the sense of virtual community in an OSS community.

%\begin{itemize}
% \item We develop a theoretical model of sense of virtual community in OSS and assess it through a survey.
% \item We examine the moderating effects of power distance and financial compensation between each of the intrinsic motivations and the sense of virtual community.
% \item We present the results of an confirmatory factor analysis of a construct to measure sense of virtual community in OSS
%\end{itemize}

% where does it come from - sense of community
%There are major uses of the term community. While geographic communities refer to a neighborhood, town, or region, relational communities involve human relationships that are not connected to a location, but communities of interest (e.g. hobby, religious, fan clubs) \cite{gusfield1975community}. 
%While numerous definitions of the term `community' exist, a common theme is that it involves human relationships based on some common characteristics. For example, geographic communities refer to a neigborhood or town where people share a place of living. Relational communities on the other hand share common interests, such as a hobby or religion \cite{gusfield1975community}. 
%Thus, a relational community is mainly conceptualized by the type of relational interactions or social ties that draw members together \cite{heller1990social}. 

%and a feeling that members have of belonging, that members matter to one another and to the group, and a shared faith that members’ needs will be met through their commitment to be together. 

%The majority of the virtual communities fall under the concept of relational communities because their members are not physically bound together \cite{hightower1998virtual}.
%Virtual groups of people interacting through electronic communication have become common within organizations and society, and can range from the professional (e.g., All of Us Research Hub) to social (e.g., Soccer enthusiasts on Yahoo groups). They can form on a variety of interactive communication technologies including mailing lists, newsgroups, chat rooms, and blogs. Although the technologies and topics vary, the members’ of these online groups share information and support \cite{jones1997virtual}. 

%, and distinguish a virtual community from other types of virtual groups \cite{blanchard2007developing} such as Honda enthusiasts on Yahoo groups, or listserv American Psychological Association of Graduate Students (APAGS). 
%While virtual groups are mostly organized to solve specific tasks and usually dissolve after the task is finished, virtual communities focus on relationship development, where people do not have definite reasons to remain in them and can exist for a very long time, as long as people with similar interests do not disperse \cite{li2004virtual}.

% how is svc measured
%Scholars have presented different versions of SVC elements. According to \cite{koh2003sense}, SVC includes the \textsc{(i) feelings of membership}, \textsc{(ii) feelings of influence} (from the sense of community), and \textsc{(iii) feelings of immersion} (feel the state of flow during virtual community navigation). Authors diverge regarding the element of \textsc{iv. integration and need fulfillment in terms of mutual support} as being part of SVC \cite{blanchard2007developing} or an expectation that precedes SVC \cite{koh2003sense,ellonen2007development,tonteri2011antecedents}. \cite{blanchard2007developing} added two more elements: \textsc{(v) feeling of identity} (feeling among the individual members of having a distinct and a common social identity with the community), and \textsc{(vi) emotional attachment} (the belief that members matter to one another and to the community).

%Over time, changes in the perceived fulfillment of contributors' instrumental, entertainment, and self-discovery needs determined the change of their SVC.

%used the metaphor of ``carrots'' for OSS contributors' motivations related to tangible, short-term, and monetary rewards, and ``rainbows'' for motivations related to intangible, long-term, social good. 
%Their review categorized OSS motivations as intrinsic, internalized-extrinsic, and extrinsic.

%Developers can also internalize extrinsic motivators in a self-regulating way so that they are perceived as internal regulation, and thus no longer requires the presence of an external contingency (e.g., working even when the boss is not watching)
%self-regulating behavior rather than external impositions \cite{taylor2022love,deci1987support,roberts2006understanding
%---these are so-called internalized extrinsic motivations \cite{gagne2005self,taylor2022love}. These motivations include reputation, reciprocity, learning, and own use.
%Most research on motivation in OSS was conducted before the professionalization of open source development, the increasing involvement of corporations, and the rise of social coding platforms such as GitHub. 

%Motivation can also be categorized as non-benefit motivations (including kinship, altruism, ideology, and reciprocity), or self-oriented and oriented to an individual contributor’s personal benefit (including fun, learn, pay, career, and reputation).

%Although diversity positively impacts OSS projects, most of the contemporary OSS projects lack diversity \cite{bosu2019diversity}. It is important for OSS projects to understand and support contributors with different motivations \cite{gerosa2021shifting}. 

%Fulfillment of needs is related to community behavior because members develop a positive sense of togetherness when their association with the group is rewarding for their motivation; 

%The kernel community needs to show that they are friendly and welcoming to everyone. Reading a single ugly or too blunt remark in an email thread is enough to do a double take if all you hear your whole life is how you don't belong in tech. And that remark doesn't even have to be directed at you - if a long term developer fitting the stereotype isn't respected, why would you?

%Even when making small contributions to projects based on their unique expertise, there is a certain degree of `ownership' that is maintained by the community of developers over time by an association of developers who wish to see the long-term survival of their project \cite{birkinbine2020incorporating}. 

%Loyalty is an attitude or cognition held by a person to characterize their relationship with another party, having implications with their levels of devotion with the organization \cite{hart2006untangling}. Embracing ideology and reciprocal obligations, loyalty also includes the sense of obligation or duty to give back to the OSS community \cite{choi2015loyalty}. 

%We draw the moderation variables upon the Cognitive Theory \cite{deci1985cognitive}, that poses feelings of autonomy are positively associated with intrinsic motivations and belonging, while tangible rewards would bring a negative effect on intrinsic factors. 

%Contributors who live in countries with high power distance cultural values tend to regard neglect by maintainers as the reasonable behavior, rather than contributors who work in countries with lower power distance.

%There are two types of SEM methods---CB-SEM and PLS-SEM---which differ in how they estimate the model parameters and in their assumptions regarding the nature of measurement. PLS-SEM emphasizes prediction and aims at maximizing the variance of endogenous latent variables by estimating partial model relationships through a sequence of ordinary least squares regressions. CB-SEM estimates model parameters in order to minimize the discrepancy between the estimated and sample covariance matrices. Instead of following a common factor model logic in estimating concept proxies as CB-SEM does, PLS-SEM calculates composites of indicators that serve as proxies for the concepts under research. The method is not constrained by identification issues, even if the model becomes complex---a situation that typically restricts CB-SEM use---and does not rely on distributional assumptions. We selected PLS-SEM because we are not going to test an existent theory in the confinement of a concise theoretical model. Our research goal is to predict and explain the sense of virtual community in the Linux Kernel.

%We followed the five steps proposed by \cite{russo2021pls}: specifying the structural model, specifying the measurement model, data collection and examining, assessing the measurement model, and assessing the structural model. Finally, we examine the moderating factors of demographics.

% Sharma (Onboarding paper)
%Research Design: 3.1. Measurement Model, 3.2. Data Collection and Analysis
%Results: 4.1. Evaluation of the Measurement Model (4.1.1. Internal Consistency Reliability, 4.1.2. Convergent Validity, 4.1.3. Discriminant Validity), 4.2. Evaluation of the Structural Model (4.2.1. Assessing Collinearity, 4.2.2. Path Coefficients and Significance, 4.2.3. Coefficient of Determination and Effect Sizes)

%We present the theoretical model in Figure \ref{fig:theoretical_model}. 


%A structural equation model is composed of a measurement model and a structural model. The structural model is the most relevant model for theory development and evaluation of hypotheses. 

%The factors were informed by the categories of intrinsic motivations from \cite{von2012carrots}'s study. To the best of our knowledge, the literature review conducted by \citet{von2012carrots} is the most comprehensive investigation of motivation in OSS, since they aggregated motivation factors found in 40 primary studies published until 2009. 

%One suggestion that we did not implement was regarding the answer options for gender identity. The participants suggested changing man per male and woman per female. We did not change because male/female refers only to the biological sex and the goal of the question is to capture whatever sex the person has/feel/changed to. 

%Besides, the demographic question about when the contributor joined the Linux Kernel had a list of years starting on 1997, and the correct start should be 1991, when the project was launched. 

%% KS MOVED TO APPENDIX
%\subsection{Common Method Bias} All data were collected through a single instrument (the survey), and methodological researchers have suggested this may lead to a systematic measurement error known as Common Method Bias (CMB) (or Common Method Variance). We tested for the presence of CMB using Harman’s single factor test [76] on the two latent variables in our model. Results showed that no factor explained more than 22\% of the variance. An exploratory factor analysis (EFA) without rotation was run with a forced single factor solution, which accounted for 28\% of variance. This is well below the maximum cut-off value of 50\%. These results indicate that common method bias was not a concern in this study
%% << END APPENDIX

%Evaluating the outer model (or measurement model) to determine how well the indicators (questions) load on the hypothetical-defined constructs is the first step in the PLS-SEM analysis \cite{hair2011pls}.

%The assessment of the reflective outer model involves the convergent validity, internal consistency reliability, and discriminant validity of the measurement model, as discussed in the following subsections.

%indicators that represent each of the two latent constructs are theoretically different ways to measure the same construct and share a considerable proportion of variance.

%As we are looking for convergence of the indicators, this shared variance must be considerable, and a rule of thumb is that this value would be at least 0.50 (so that at least half of the variance is shared across indicators). 

%Considering the loadings should be at least the square root of 0.5 (which is 0.708), a outer loading of 0.7 is widely considered sufficient \cite{hair2019use}.

%except one with .60 (\textit{svc4: I want to contribute more but I do not feel valued}). However, retaining this indicator did not have any negative effect on the discriminant validity (discussed below). Following Hair et al. and given the exploratory nature of the model, and that the loading was .6, we decided to keep this indicator.

%We evaluated the discriminant validity through three procedures.
%can be evaluated by using cross-loading of indicator, Fornell-Larcker criterion, and Heterotrait-monotrait (HTMT) ratio of correlation.

%\textit{Heterotrait-Monotrait (HTMT) ratio:} 
%In addition, HTMT ratios should also be significantly different from 1.0; this can be calculated using a bootstrap procedure, which calculates bias-corrected confidence intervals for all ratios.

%Other procedures exist to assess discriminant validity: assessing cross-loadings of indicators and the assessment of the Fornell-Larcker criterion. However, both procedures have been shown to be insufficient and are now considered obsolete.

%\textit{Cross-loading of indicators:} The indicators' loadings should be higher for the constructs they purportedly measure than for other constructs. If an indicator loads higher onto a different construct than the one that it purportedly measures, the indicator may be a better measure for that other construct. The two latent variables have indicators that load highest onto their respective constructs.

%\input{Tables/cross_loadings}

%\textit{Fornell-Larcker criterion:} According to this criterion, the square root of a construct’s AVE should be higher than that construct’s correlation with other constructs. This means that a construct should share more variance with its own indicators than with other constructs. We observed that the AVE value for SVC was 0.746 (approx. three times higher than the correlation with English Confidence). Table \ref{tab:new_fornell_larcker} lists the construct correlations, with the square roots of the AVE values on the diagonal. All square roots of the AVE values comply with the Fornell-Larcker criterion.

%\input{Tables/new_fornell_larcker}


%Figure \ref{fig:evaluating_structutal_model}} shows that the direct association between kinship/altruism and fun motivations to sense of virtual community are significant (p=xxx). On the other hand, ideology/reciprocity association with a sense of virtual community is not statistically significant (p-xxx). Section \ref{sec:discussion} presents a discussion of these results.

%\includegraphics[width=0.7\textwidth]{Figures/evaluating_structural_model.pdf}
%% KS made modifications. broke the golden left-to-right rule, but (1) nobody in SE knows about that, (2) they're control vars, and (3) needs must. (no space!)

%The value of $R^{2}$ will change when an exogenous construct is removed from the model—a measure for the extent to which the exogenous construct contributes to an endogenous construct's $R^{2}$ value is the $f^{2}$ effect size. Table \ref{tab:effect_size} lists the $f^{2}$ values for each of the constructs. 
%As suggested by \cite{cohen1992statistical}, if the value of $f^{2}$ is less than 0.02, it indicates that there is no effect of the exogenous construct on the endogenous construct. This study shows that there is an effect for H1, H2, H4a, H5b, and the three control variables. %An effect size below 0.02 means that there is no effect of the exogenous construct on the endogenous construct. The threshold values 0.02, 0.15, and 0.35 refer to, respectively, small, medium, and large effects \cite{cohen1992statistical}. 
%The table shows that of the constructs associated with SVC, \textsc{Tenure} have a small effect but makes the largest contribution to the $R^{2}$ with an $f^{2}$ effect size of approximately 0.08, followed by the Fun and Kinship motivations, also with small effects, but contributing to the $R^{2}$ with an $f^{2}$ effect size of approximately 0.06 and 0.04, respectively.

%While comparing the \textit{Q}\textsuperscript{2} value to zero is indicative of whether an endogenous latent variable can be predicted, it does not say anything about the quality of the prediction. In analogy to the ƒ² effect size, researchers can compute the q2 effect size, which allows for evaluating the relative impact of one construct in terms of its predictive relevance.

%In analogy to the $f^{2}$ effect size, researchers can compute the $Q^{2}$ effect size, which allows for evaluating the relative impact of one construct in terms of its predictive relevance. The same thresholds as for the $f^{2}$ apply to $Q^{2}$ (0.02, 0.15, 0.35). The $Q^{2}$ value shows that our model has a medium predictive relevance.

%For all variables we examined if there were any correlations with (other) demographic and sense of virtual community variable. We then treated each variable as a moderating effect in the model. 

%The segmentation goal of PLS-POS is to form homogeneous groups of observations with increased predictive power in terms of {R}\textsuperscript{2} of the endogenous latent variable (compared to the overall sample model). A fitting objective criterion for PLS segmentation is to maximize the sum of the endogenous latent variables' explained variance ({R}\textsuperscript{2}) across all group by taking the entire path model's structure into account. POS-PLS reassigns observations only if reassigning observations improves the objective criterion, interacting the algorithm (hill-climbing approach) and providing the ability to uncover very small niche segments \cite{becker2013discovering}.

%

%PLS-POS follows a clustering approach with a deterministic assignment of observations to groups and uses a distance measure for the reassignment of observations; as such, it has no distributional assumptions. 

%The PLS-POS method uses a distance measure to identify appropriate observations for reassignment that serve as candidates to improve the PLS-POS objective criterion. Using a distance measure (i.e., calculating each observation's distance from its current group and from each of the other groups) for segmentation builds on an idea of earlier work on distance-measure-based segmentation in PLS path modeling (i.e., PLS-TPM and its later improvement REBUS-PLS).
% The PLS-POS method complies with the most relevant goals in PLS path modeling. It (1) improves the objective criterion by nonparametric means; (2) accounts for heterogeneity in the structural model, as well as in the formative measurement model; and (3) is applicable to all path models regardless of the type of measurement model, the distribution of the data, or the complexity of the structural mode.
%FIMIX-PLS allows the simultaneous estimation of model parameters and segment affiliations of observations \cite{sarstedt2008review}, relying in finite mixture approach and assuming that the data originate from several subpopulations (segments) \cite{mclachlan2004finite}. Each segment is modeled separately and the overall population is a mixture of the segments.

%FIMIX-PLS calculates the probability of belonging to any given segment in which each observation is adjusted to the predetermined number of segments by estimating separate linear regression functions, which gives a group of possible segments \cite{hair2016identifying}.

%\subsubsection{Uncovering unobserved heterogeneity}

%(e.g., Akaike (AIC) and Akaike Modified AIC with Factor 3 (AIC3) and Factor 4 (AIC4), the Consistent AIC (CAIC), the Bayesian information criteria (BIC), Minimum Description Length with Factor 5 (MDL5), and the standardized entropy statistic (EN))

%The step to to approximate the best fitting number of segments includes defining with heuristics a range of statistically well-fitting segments from finite mixture modeling literature (e.g., Akaike (AIC) and Akaike Modified AIC with Factor 3 (AIC3) and Factor 4 (AIC4), the Consitent AIC (CAIC), the Bayesian information criteria (BIC), Minimum Description Length with Factor 5 (MDL5), and the standardized entropy statistic (EN)) \cite{sarstedt2008review}.

%The online appendix provides a complete overview of the selection criteria for unobserved segmentation analysis \cite{replication_package}.

%Although the GoF for the PLS–SEM should not be used as an indicator of fit, it is considered useful for comparing results in a multi-group analysis (MGA), especially for unobserved heterogeneity \cite{henseler2013goodness}.

%Besides online interest groups for members, chat rooms, instant messaging, and discussion forums to encourage community involvement \cite{xu2015empirical}, OSS communities can provide online tools with shared spaces for contributors to work ``together" on issues, discuss and collaborate on similar interests. Better interactions can strengthen contributors’ Sense of Virtual Community, especially for those who seek social relationships. When the information being exchanged surpasses the technical content and include also socio-emotional support, it can evidence personal relationships among group members, and finally bring feelings of acceptance by members \cite{blanchard2011sense}. OSS communities should foster exchanging support among members to bring a positive impact on developing SVC \cite{tonteri2011antecedents}. The exchanging support includes both technical and social support and happens through comments in pull requests and participation in mailing lists (by either reading or posting messages). Communities can manage pull requests and mailing lists to guarantee that members' posts are not being missed \cite{miller2022did}, while the communication is being adherent to the code of conduct.

%Table \ref{tab:discussion} provides a summary.

%\input{Tables/discussion}

%We found support for H1 which proposed a positive association between contributors motivated by the social motives of kinship or altruism to experience a sense of virtual community.

%\textbf{Foster a sense of virtual community among OSS contributors.} 
%OSS communities should foster exchanging support among members to bring a positive impact on developing SVC \cite{tonteri2011antecedents}. The exchanging support includes both technical and social support, and happen through comments in pull requests and participation in mailing lists (by either reading or posting messages). Communities can manage pull-requests and mailing lists to guarantee that members' posts are not being missed \cite{miller2022did}, while the communication is being adherent to the code of conduct. When the information being exchanged surpasses the technical content and include also socio-emotional support, it can evidence personal relationships among group members, and finally bring feelings of acceptance by members \cite{blanchard2011sense}. Members participate in the community through exchanging information, providing support, and observing others provide support, they develop more positive feelings toward the community and a stronger attachment to it. \cite{blanchard2004experienced}. Lurking is a valuable form of participation in virtual communities \cite{tonteri2011antecedents} and in OSS \cite{trinkenreich2020hidden}. Making the input of lurkers visible through ratings and voting tools, for example, can incentive this activity and lead to the development of SVC \cite{tonteri2011antecedents}. When not exerted in toxic and harsh ways to discipline community members, concertive control can also ultimately play a prosocial role in increasing the SVC, by increasing cohesiveness, commitment, and conformity \cite{gibbs2019investigating}. 

%When the intrinsic motivation factors and personal characteristics of an individual do not ``fit" with a community, it negatively affect their feelings of belonging \cite{sax2018sense}. The project page can have cues that match (and improve) or mismatch (and impede) contributors' "fit" of their motivations and the project. For example, if the project uses leaderboards to highlight individuals who close the most issues or make the most commits (a mechanism that exists on GitHub), it promotes competition rather than kinship. These are just two examples where the project landscape can match (and improve) or mismatch (and impede) contributors' "fit," and consequently their sense of belonging.

 
%\textit{Promote mutual trust.} People who communicate electronically with unknown others are understandably concerned whether the others actually are who they say they are, specially when members aim to develop social connections.

%The use of PLS-POS with FIMIX is considered more beneficial for treating unobserved heterogeneity and is applicable regardless of the mode of the measurement model, data distribution, or complexity of the structural model. 

%Therefore, considering the sense of virtual community as a concept that brings social support, we aim to investigate this concept as an additional force that can influence the contributor's decision to remain in an OSS project. 
